Self-Evolving Neuro-Symbolic Skills for Tool-Augmented Spatial Reasoning

Large vision-language models have achieved strong performance in multimodal reasoning, but they remain unreliable on fine-grained spatial tasks that demand both precise spatial perception and fine-grained geometric computation beyond end-to-end generation. Tool augmentation offers a natural solution, while existing methods either plan tool calls from scratch without explicit dependency constraints or rely on fixed pipelines that are redundant and generalize poorly across spatial tasks. An effective spatial reasoning agent should instead accumulate reusable experience and adaptively compose it for new problems. To this end, we propose NeSy-Spatial, a neuro-symbolic framework for self-evolving spatial skills. NeSy-Spatial abstracts tool interactions and geometric operations into typed executable atomic instructions and composes them into two complementary skill types: Tool-Use Skills for organizing tool execution and Geometry Skills for structured geometric reasoning. During inference, NeSy-Spatial retrieves and executes relevant skills in a closed-loop process. During evolution, it analyzes buffered successful and failed trajectories to refine skill structures and prune unreliable or inactive entries. Experiments on three spatial reasoning benchmarks show that NeSy-Spatial consistently improves reasoning accuracy with more precise tool utilization.

==> Tables/RQ2_tool_compact.tex <==
% Compact main-text version of the tool-use reliability table.
\begin{table}[t]
\centering
\small
\caption{
Compact comparison of tool-use reliability under GPT and Gemini.
FTCS measures compositional tool-flow correctness, and Python success rate measures successful Python executions.
Dashes indicate pending results.
}
\label{tab:tool_reliability_compact}
\setlength{\tabcolsep}{4pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
& \multicolumn{2}{c}{FTCS $\uparrow$}
& \multicolumn{2}{c}{Python Success Rate $\uparrow$} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
Method
& GPT & Gemini
& GPT & Gemini \\
\midrule
SpaAge-PE
& -- & -- & -- & -- \\

SpaAge-ReAct
& -- & -- & -- & -- \\

AWM
& -- & -- & -- & -- \\

ASI
& -- & -- & -- & -- \\

GCA
& -- & -- & -- & -- \\

\textsc{NeSy-Spatial}
& -- & -- & -- & -- \\
\bottomrule
\end{tabular}
}
\end{table}

